ST-VLM: Kinematic Instruction Tuning for Spatio-Temporal Reasoning in Vision-Language Models

Spatio-temporal reasoning is essential in understanding real-world environments in various fields, eg, autonomous driving and sports analytics. Recent advances have improved the spatial reasoning ability of Vision-Language Models (VLMs) by introducing large-scale data, but these models still struggle to analyze kinematic elements like traveled distance and speed of moving objects. To bridge this gap, we construct a spatio-temporal reasoning dataset and benchmark involving kinematic instruction tuning, referred to as STKit and STKit-Bench. They consist of real-world videos with 3D annotations, detailing object motion dynamics: traveled distance, speed, movement direction, inter-object distance comparisons, and relative movement direction. To further scale such data construction to videos without 3D labels, we propose an automatic pipeline to generate pseudo-labels using 4D reconstruction in real-world scale. With our kinematic instruction tuning data for spatio-temporal reasoning, we present ST-VLM, a VLM enhanced for spatio-temporal reasoning, which exhibits outstanding performance on STKit-Bench. Furthermore, we show that ST-VLM generalizes robustly across diverse domains and tasks, outperforming baselines on other spatio-temporal benchmarks (eg, ActivityNet, TVQA+). Finally, by integrating learned spatio-temporal reasoning with existing abilities, ST-VLM enables complex multi-step reasoning. Project page: https://ikodoh.github.io/ST-VLM.

==> Figures/challenging/challenging.tex <==
\begin{figure*}[!t] 
    \centering
    \begin{subfigure}[h]{0.49\linewidth}
        \includegraphics[width=1.0\linewidth]{Figures/challenging/challenging1.pdf}
        \caption{}
        \label{fig:challenging1}
    \end{subfigure}
    \begin{subfigure}[h]{0.49\linewidth}
        \includegraphics[width=1.0\linewidth]{Figures/challenging/challenging2.pdf}
        \caption{}
        \label{fig:challenging2}
    \end{subfigure}
    \begin{subfigure}[h]{0.49\linewidth}
        \includegraphics[width=1.0\linewidth]{Figures/challenging/challenging3.pdf}
        \caption{}
        \label{fig:challenging3}
    \end{subfigure}
    \begin{subfigure}[h]{0.49\linewidth}
        \includegraphics[width=1.0\linewidth]{Figures/challenging/challenging4.pdf}
        \caption{}
        \label{fig:challenging4}
    \end{subfigure}
    \caption{\textbf{Further qualitative results on challenging examples.}}
    \label{fig:challenging}
\end{figure*}

==> Figures/emerging/emerging.tex <==
\begin{figure}[ht] 
    \centering
    \begin{subfigure}[h]{\linewidth}
        \includegraphics[width=1.0\linewidth]{Figures/emerging/emerging.pdf}
        % \caption{Traveled Distance}
    \end{subfigure}
    \caption{\textbf{Qualitative results of emerging capabilities.}}
    \label{fig:emerging}
\end{figure}

==> Figures/intro/intro_ori.tex <==
\begin{center}
    \centering
    \captionsetup{type=figure}
    \begin{subfigure}[b]{\textwidth}
        \centering
        \includegraphics[width=0.98\textwidth]{Figures/intro/intro1.pdf}
        \caption{ }
        \label{fig:intro1}
    \end{subfigure}
    \begin{subfigure}[b]{0.49\textwidth}
        \includegraphics[width=\textwidth]{Figures/intro/intro2.pdf}
        \caption{}
        \label{fig:intro2}
    \end{subfigure}
    \begin{subfigure}[b]{0.49\textwidth}
        \includegraphics[width=\textwidth]{Figures/intro/intro3.pdf}
        \caption{}
        \label{fig:intro3}
    \end{subfigure}
    \caption{
    Given dynamic videos of moving objects, these are examples of spatio-temporal reasoning:
    (a) \textbf{Video-question pairs from the proposed STKit-Bench along with predictions from ST-VLM}.
    (b) \textbf{A challenging example with a complex trajectory}, asking for the traveled distance for a basketball player moves erratically across the court. 
    (c) \textbf{An emerging capabilities of ST-VLM involving multi-step reasoning}, \eg, distance retrieval, speed estimation, and time calculation. 
    In both (b) and (c), GPT-4V struggles with advanced spatio-temporal reasoning, whereas ST-VLM consistently provides accurate answers.
    }
    \label{fig:intro}
\end{center}

==> Figures/perception.tex <==
\begin{figure}[t] 
    \centering
    \includegraphics[width=\linewidth]{Figures/perception.pdf}
    \caption{\textbf{Qualitative example on PerceptionTest.}
    Blue signifies the accurate prediction, while red denotes the incorrect prediction.
    }
    \label{fig:perception}
\end{figure}

==> Figures/perception/perception.tex <==
\begin{figure*}[!t] 
    \centering
    \begin{subfigure}[h]{0.49\linewidth}
        \includegraphics[width=1.0\linewidth]{Figures/perception/perception2.pdf}
        \caption{}
        \label{fig:perception1}
    \end{subfigure}
    \begin{subfigure}[h]{0.49\linewidth}
        \includegraphics[width=1.0\linewidth]{Figures/perception/perception1.pdf}
        \caption{}
        \label{fig:perception2}
    \end{subfigure}
    \caption{\textbf{Qualitative results on PerceptionTest.}
    Blue signifies the accurate prediction, while red denotes the incorrect prediction.}
    \label{fig:perception}
\end{figure*}

==> Figures/stkit_bench/stkit_bench.tex <==
\begin{figure*}[!t] 
    \centering
    \begin{subfigure}[h]{0.49\linewidth}
        \includegraphics[width=1.0\linewidth]{Figures/stkit_bench/distance.pdf}
        \caption{Traveled Distance}
        \label{fig:distance}
    \end{subfigure}
    \begin{subfigure}[h]{0.49\linewidth}
        \includegraphics[width=1.0\linewidth]{Figures/stkit_bench/speed.pdf}
        \caption{Traveling Speed}
        \label{fig:speed}
    \end{subfigure}
    \begin{subfigure}[h]{0.49\linewidth}
        \includegraphics[width=1.0\linewidth]{Figures/stkit_bench/direction.pdf}
        \caption{Movement Direction}
        \label{fig:direction}
    \end{subfigure}
    \begin{subfigure}[h]{0.49\linewidth}
        \includegraphics[width=1.0\linewidth]{Figures/stkit_bench/timestamp.pdf}
        \caption{Direction Timestamp}
        \label{fig:timestamp}
    \end{subfigure}
    \caption{\textbf{Qualitative results on STKit-Bench.}}
    \label{fig:stkit_bench1}
\end{figure*}

\begin{figure*}[!t] 
    \centering
    \begin{subfigure}[h]{0.49\linewidth}
        \includegraphics[width=1.0\linewidth]{Figures/stkit_bench/distance_comparison.pdf}
        \caption{Traveled Distance Comparison}
        \label{fig:distance_comparison}
    \end{subfigure}
    \begin{subfigure}[h]{0.49\linewidth}
        \includegraphics[width=1.0\linewidth]{Figures/stkit_bench/speed_comparison.pdf}
        \caption{Traveling Speed Comparison}
        \label{fig:speed_comparison}
    \end{subfigure}
    \begin{subfigure}[h]{0.49\linewidth}
        \includegraphics[width=1.0\linewidth]{Figures/stkit_bench/direction_comparison.pdf}
        \caption{Movement Direction Comparison}
        \label{fig:direction_comparison}
    \end{subfigure}
    \caption{\textbf{Qualitative results on STKit-Bench.}}
    \label{fig:stkit_bench2}
\end{figure*}

==> Figures/trajectory/trajectory.tex <==
\begin{figure}[!ht] 
    \centering
    \begin{subfigure}[h]{0.49\linewidth}
        \includegraphics[width=1.0\linewidth]{Figures/trajectory/trajectory1.pdf}
        \caption{}
        \label{fig:trajectory1}
    \end{subfigure}
    \begin{subfigure}[h]{0.49\linewidth}
        \includegraphics[width=1.0\linewidth]{Figures/trajectory/trajectory2.pdf}
        \caption{}
        \label{fig:trajectory2}
    \end{subfigure}
    \caption{\textbf{Comparison of projected trajectories.} 
    GT trajectory is shown in \textcolor{gray}{grey dash line} and estimated trajectory from pseudo-label (PS) is shown in \textcolor{blue}{blue solid line}.}
    \label{fig:trajectory}
\end{figure}

==> Figures/trajectory/trajectory_vert.tex <==
\begin{figure}[t!]
    \centering
    \includegraphics[width=\linewidth]{Figures/traj_comb.png}
    \caption{\textbf{Trajectory 1.}}
    \label{fig:traj}
\end{figure}

==> Tables/domain.tex <==
% \begin{table}[!t]
%     \centering
%     % \begin{adjustbox}{width=\linewidth}
%     % \setlength{\tabcolsep}{4.0pt}
%     \scriptsize
%     \begin{tabular}{c c||c c|c c}
%         \toprule
%         \multirow{2}{*}{\textbf{Train}} & \multirow{2}{*}{\textbf{Test}} & \multicolumn{2}{c|}{\textbf{Traveled Distance}} & \multicolumn{2}{c}{\textbf{Traveling Speed}} \\
%         & & Acc$\uparrow$ & MAE$\downarrow$ & Acc$\uparrow$ & MAE$\downarrow$ \\
%         \midrule
%         \midrule
%         - & Sports & 16.0 & 6.7 & 8.0 & 2.8 \\
%         Sports & Sports & \textbf{76.0} & 2.0 & \textbf{78.0} & 0.8 \\
%         \rowcolor{aliceblue}
%         AD + Sports & Sports & \textbf{76.0} & \textbf{1.7} & \textbf{78.0} & \textbf{0.7} \\
%         \bottomrule
%     \end{tabular}
%     % \end{adjustbox}
%     \caption{\textbf{Quantitative analysis on different domains.}
%     AD stands for autonomous driving.
%     }
%     \label{tab:domain}
% \end{table}


\begin{table}[!h]
    \centering
    % \begin{adjustbox}{width=\linewidth}
    % \setlength{\tabcolsep}{4.0pt}
    \scriptsize
    \begin{tabular}{c c||c c|c c}
        \toprule
        \multirow{2}{*}{\textbf{Train}} & \multirow{2}{*}{\textbf{Test}} & \multicolumn{2}{c|}{\textbf{Traveled Distance}} & \multicolumn{2}{c}{\textbf{Traveling Speed}} \\
        & & Acc$\uparrow$ & MAE$\downarrow$ & Acc$\uparrow$ & MAE$\downarrow$ \\
        \midrule
        \midrule
        - & Sports & 16.0 & 6.7 & 8.0 & 2.8 \\
        AD & Sports & 22.0 & 4.8 & 64.0 & 0.9 \\
        Sports & Sports & \textbf{76.0} & 2.0 & \textbf{78.0} & 0.8 \\
        \rowcolor{aliceblue}
        AD + Sports & Sports & \textbf{76.0} & \textbf{1.7} & \textbf{78.0} & \textbf{0.7} \\
        \midrule
        - & AD & 13.0 & 49.1 & 10.0 & 24.3 \\
        AD & AD & 35.5 & 21.7 & 32.0 & \textbf{12.6} \\
        Sports & AD & 5.0 & 36.4 & 6.5 & 29.0 \\
        \rowcolor{aliceblue}
        AD + Sports & AD & \textbf{38.5} & \textbf{17.0} & \textbf{32.5} & \textbf{12.6} \\
        \bottomrule
    \end{tabular}
    % \end{adjustbox}
    \caption{\textbf{Quantitative results on each domain of STKit-Bench.}
    AD stands for autonomous driving. 
    The row where the \textbf{Train} column is marked with "-" corresponds to the baseline LLaVA-OneVision~\cite{li2024llava}. 
    }
    \label{tab:domain}
\end{table}

==> Tables/prompts/direction_timestamp.tex <==
\begin{table*}[!t]\centering

\begin{minipage}{0.99\linewidth}\vspace{0mm}    \centering
\begin{tcolorbox} 
    \centering
    \small
     \hspace{-6mm}
    \begin{tabular}{p{0.99\linewidth}}

\begin{minipage}{0.99\linewidth}\vspace{0mm}

\VarSty{direction\_timestamp\_prompt} \var{= f"""}You should help me to evaluate the response given the question and the correct answer.

You need to extract the start time and end time in seconds of the correct answer and response.

You should output two Python Tuples with the format of '(start, end)', one for the answer, and 
one for the response.

The output should be in JSON format.\var{"""} \\

\VarSty{messages} = [
            \{\var{"role":"system", "content":direction\_timestamp\_prompt}\}]
        
    \For{ \VarSty{sample} in   \VarSty{fewshot\_samples}}{
         \var{\VarSty{messages}.append(\{"role":"user", "content":\VarSty{sample[`context']}\})} \; \\
         \var{\VarSty{messages}.append(\{"role":"assistant", "content":\VarSty{sample[`response']}\}) } \;
         }  
    \var{\VarSty{messages}.append(\{"role":"user", "content":`\textbackslash  n'.join(\VarSty{query})\})}
\end{minipage}
    \end{tabular}
\end{tcolorbox}
    
\vspace{-2mm}
\caption{\textbf{GPT-4 prompts for Direction Timestamp.}}
    \label{tab:direction_timestamp_prompt}
\end{minipage}
\end{table*}

==> Tables/prompts/movement_direction.tex <==
\begin{table*}[!t]\centering

\begin{minipage}{0.99\linewidth}\vspace{0mm}    \centering
\begin{tcolorbox} 
    \centering
    \small
     \hspace{-6mm}
    \begin{tabular}{p{0.99\linewidth}}

\begin{minipage}{0.99\linewidth}\vspace{0mm}

\VarSty{movement\_direction\_prompt} \var{= f"""}You should help me to evaluate the response given the question and the correct answer.

You need to extract the direction of the correct answer and response.

You should output two integers in clock directions, one for the answer, and one for the response.

The output should be in JSON format.\var{"""} \\

\VarSty{messages} = [
            \{\var{"role":"system", "content":movement\_direction\_prompt}\}]
        
    \For{ \VarSty{sample} in   \VarSty{fewshot\_samples}}{
         \var{\VarSty{messages}.append(\{"role":"user", "content":\VarSty{sample[`context']}\})} \; \\
         \var{\VarSty{messages}.append(\{"role":"assistant", "content":\VarSty{sample[`response']}\}) } \;
         }  
    \var{\VarSty{messages}.append(\{"role":"user", "content":`\textbackslash  n'.join(\VarSty{query})\})}
\end{minipage}
    \end{tabular}
\end{tcolorbox}
    
\vspace{-2mm}
\caption{\textbf{GPT-4 prompts for Movement Direction.}}
    \label{tab:movement_direction_prompt}
\end{minipage}
\end{table*}

==> Tables/prompts/movement_direction_comparison.tex <==
\begin{table*}[!t]\centering

\begin{minipage}{0.99\linewidth}\vspace{0mm}    \centering
\begin{tcolorbox} 
    \centering
    \small
     \hspace{-6mm}
    \begin{tabular}{p{0.99\linewidth}}

\begin{minipage}{0.99\linewidth}\vspace{0mm}

\VarSty{movement\_direction\_comparison\_prompt} \var{= f"""}You should help me to evaluate the response given the question and the correct answer.

To mark a response, you should output a single integer between 0 and 1.

1 means that the response perfectly matches the answer.

0 means that the response is completely different from the answer.

The output should be in JSON format.\var{"""} \\

\VarSty{messages} = [
            \{\var{"role":"system", "content":movement\_direction\_comparison\_prompt}\}]
        
    \For{ \VarSty{sample} in   \VarSty{fewshot\_samples}}{
         \var{\VarSty{messages}.append(\{"role":"user", "content":\VarSty{sample[`context']}\})} \; \\
         \var{\VarSty{messages}.append(\{"role":"assistant", "content":\VarSty{sample[`response']}\}) } \;
         }  
    \var{\VarSty{messages}.append(\{"role":"user", "content":`\textbackslash  n'.join(\VarSty{query})\})}
\end{minipage}
    \end{tabular}
\end{tcolorbox}
    
\vspace{-2mm}
\caption{\textbf{GPT-4 prompts for Movement Direction Comparison.}}
    \label{tab:movement_direction_comparison_prompt}
\end{minipage}
\end{table*}

==> Tables/prompts/traveled_distance.tex <==
\begin{table*}[!t]\centering

\begin{minipage}{0.99\linewidth}\vspace{0mm}    \centering
\begin{tcolorbox} 
    \centering
    \small
     \hspace{-6mm}
    \begin{tabular}{p{0.99\linewidth}}

\begin{minipage}{0.99\linewidth}\vspace{0mm}

\VarSty{traveled\_distance\_prompt} \var{= f"""} You are a helpful assistant designed to output JSON.

You should help me to evaluate the response given the question and the correct answer.

You need to convert the distance of the correct answer and response to meters. 

The conversion factors are as follows: 1 inch = 0.0254 meters. 1 foot = 0.3048 meters. 1 centimeter (cm) = 0.01 meters.

You should output two floats in meters, one for the answer, and one for the response.

The output should be in JSON format.\var{"""} \\

\VarSty{messages} = [
            \{\var{"role":"system", "content":traveled\_distance\_prompt}\}]
        
    \For{ \VarSty{sample} in   \VarSty{fewshot\_samples}}{
         \var{\VarSty{messages}.append(\{"role":"user", "content":\VarSty{sample[`context']}\})} \; \\
         \var{\VarSty{messages}.append(\{"role":"assistant", "content":\VarSty{sample[`response']}\}) } \;
         }  
    \var{\VarSty{messages}.append(\{"role":"user", "content":`\textbackslash  n'.join(\VarSty{query})\})}
\end{minipage}
    \end{tabular}
\end{tcolorbox}
    
\vspace{-2mm}
\caption{\textbf{GPT-4 prompts for Traveled Distance.}}
    \label{tab:traveled_distance}
\end{minipage}
\end{table*}

==> Tables/prompts/traveled_distance_comparison.tex <==
\begin{table*}[!t]\centering

\begin{minipage}{0.99\linewidth}\vspace{0mm}    \centering
\begin{tcolorbox} 
    \centering
    \small
     \hspace{-6mm}
    \begin{tabular}{p{0.99\linewidth}}

\begin{minipage}{0.99\linewidth}\vspace{0mm}

\VarSty{traveled\_distance\_comparison\_prompt} \var{= f"""}You should help me to evaluate the response given the question and the correct answer.

To mark a response, you should output a single integer between 0 and 1.

1 means that the response perfectly matches the answer.

0 means that the response is completely different from the answer.

The output should be in JSON format.\var{"""} \\

\VarSty{messages} = [
            \{\var{"role":"system", "content":traveled\_distance\_comparison\_prompt}\}]
        
    \For{ \VarSty{sample} in   \VarSty{fewshot\_samples}}{
         \var{\VarSty{messages}.append(\{"role":"user", "content":\VarSty{sample[`context']}\})} \; \\
         \var{\VarSty{messages}.append(\{"role":"assistant", "content":\VarSty{sample[`response']}\}) } \;
         }  
    \var{\VarSty{messages}.append(\{"role":"user", "content":`\textbackslash  n'.join(\VarSty{query})\})}
\end{minipage}
    \end{tabular}
\end{tcolorbox}
    
\vspace{-2mm}
\caption{\textbf{GPT-4 prompts for Traveled Distance Comparison.}}
    \label{tab:traveled_distance_comparison_prompt}
\end{minipage}
\end{table*}

==> Tables/prompts/traveling_speed.tex <==
\begin{table*}[!t]\centering

\begin{minipage}{0.99\linewidth}\vspace{0mm}    \centering
\begin{tcolorbox} 
    \centering
    \small
     \hspace{-6mm}
    \begin{tabular}{p{0.99\linewidth}}

\begin{minipage}{0.99\linewidth}\vspace{0mm}

\VarSty{traveling\_speed\_prompt} \var{= f"""}You should help me to evaluate the response given the question and the correct answer.

You need to convert the speed of the correct answer and response to kilometers per hour (km/h). 
The conversion factors are as follows: 1 meters per second (m/s) = 3.6 kilometers per hour (km/h). 

1 miles per hour (mph) = 1.60934 kilometers per hour (km/h). 1 foot per second (ft/s) = 1.09728 kilemoeters per hour (km/h).

You should output two floats in kilometers per hour (km/h), one for the answer, and one for the response.

The output should be in JSON format.\var{"""} \\

\VarSty{messages} = [
            \{\var{"role":"system", "content":traveling\_speed\_prompt}\}]
        
    \For{ \VarSty{sample} in   \VarSty{fewshot\_samples}}{
         \var{\VarSty{messages}.append(\{"role":"user", "content":\VarSty{sample[`context']}\})} \; \\
         \var{\VarSty{messages}.append(\{"role":"assistant", "content":\VarSty{sample[`response']}\}) } \;
         }  
    \var{\VarSty{messages}.append(\{"role":"user", "content":`\textbackslash  n'.join(\VarSty{query})\})}
\end{minipage}
    \end{tabular}
\end{tcolorbox}
    
\vspace{-2mm}
\caption{\textbf{GPT-4 prompts for Traveling Speed.}}
    \label{tab:traveling_speed_prompt}
\end{minipage}
\end{table*}

==> Tables/prompts/traveling_speed_comparison.tex <==
\begin{table*}[!t]\centering

\begin{minipage}{0.99\linewidth}\vspace{0mm}    \centering
\begin{tcolorbox} 
    \centering
    \small
     \hspace{-6mm}
    \begin{tabular}{p{0.99\linewidth}}

\begin{minipage}{0.99\linewidth}\vspace{0mm}

\VarSty{traveling\_speed\_comparison\_prompt} \var{= f"""}You should help me to evaluate the response given the question and the correct answer.

To mark a response, you should output a single integer between 0 and 1.

1 means that the response perfectly matches the answer.

0 means that the response is completely different from the answer.

The output should be in JSON format.\var{"""} \\

\VarSty{messages} = [
            \{\var{"role":"system", "content":traveling\_speed\_comparison\_prompt}\}]
        
    \For{ \VarSty{sample} in   \VarSty{fewshot\_samples}}{
         \var{\VarSty{messages}.append(\{"role":"user", "content":\VarSty{sample[`context']}\})} \; \\
         \var{\VarSty{messages}.append(\{"role":"assistant", "content":\VarSty{sample[`response']}\}) } \;
         }  
    \var{\VarSty{messages}.append(\{"role":"user", "content":`\textbackslash  n'.join(\VarSty{query})\})}
\end{minipage}
    \end{tabular}
\end{tcolorbox}
    
\vspace{-2mm}
\caption{\textbf{GPT-4 prompts for Traveling Speed Comparison.}}
    \label{tab:traveling_speed_comparison_prompt}
\end{minipage}
\end{table*}

==> Tables/templates/direction.tex <==
\begin{figure*}[t]
\begin{lstlisting}[basicstyle=\ttfamily\small, backgroundcolor = \color{lightgray}, keywordstyle = {\textbf}, caption={\textbf{QA templates for Movement Direction.}}, label={list:md}, breaklines=true]
movement_direction_common_prompt = f"""The video lasts for [SECONDS] seconds, and [FRAMES] 
frames are uniformly sampled from it. These frames are located at [SECOND1]s,[SECOND2]s,
[SECOND3]s, ... . Please answer the following questions related to this video.

There is an object annotated with a [COLOR] bounding box in the video.
"""

movement_direction_questions = [
    "In which direction does the object move at the end of the video?",
    "What direction does the object travel at the end of the video?",
    "At the end of the video, in which direction does the object move?",
    "Describe the direction of the object moving at the end of the video",
    "Provide the direction of the object moving at the end of the video."
]

movement_direction_answers = [
    "The given object is heading toward the [CLOCK] o'clock direction at the end of the 
    video.",
    "The object moves in the direction of [CLOCK] o'clock at the end of the video.",
    "At the end of the video, the object is heading toward the [CLOCK] o'clock direction.",
    "The object is traveling toward the [CLOCK] o'clock direction at the end of the video.",
    "At the end of the video, the object moves toward the [CLOCK] o'clock direction."
]
\end{lstlisting}
\end{figure*}

==> Tables/templates/direction_comparison.tex <==
\begin{figure*}[t]
\begin{lstlisting}[basicstyle=\ttfamily\small, backgroundcolor = \color{lightgray}, keywordstyle = {\textbf}, caption={\textbf{Question templates for Movement Direction Comparison.}}, label={list:mdc_q}, breaklines=true]
movement_direction_comparison_common_prompt = f"""The video lasts for [SECONDS] seconds, 
and [FRAMES] frames are uniformly sampled from it. These frames are located at [SECOND1]s,
[SECOND2]s,[SECOND3]s, ... . Please answer the following questions related to this video.

There are two objects annotated with [COLOR1] and [COLOR2] bounding boxes in the video.
"""


movement_direction_comparison_positive_questions = [
    "Is the object annotated with the [COLOR1] bounding box moving in the same direction as 
    the object annotated with the [COLOR2] bounding box in the video?",
    "Is the object annotated with the [COLOR1] bounding box heading in the same direction 
    as the object annotated with the [COLOR2] bounding box throughout the video?",
    "Are the object annotated with the [COLOR1] bounding box and the object annotated with 
    the [COLOR2] bounding box moving in the same direction during the video?",
    "In the video, does the object with the [COLOR1] bounding box move in the same 
    direction as the object with the [COLOR2] bounding box?",
    "Are the objects annotated with the [COLOR1] and [COLOR2] bounding boxes traveling in 
    the same direction during the entire video?"
]

movement_direction_comparison_negative_questions = [
    "Is the object annotated with the [COLOR1] bounding box moving in a different direction 
    from the object annotated with the [COLOR2] bounding box in the video?",
    "Is the object annotated with the [COLOR1] bounding box heading in a different 
    direction from the object annotated with the [COLOR2] bounding box from throughout the 
    video?",
    "Are the object annotated with the [COLOR1] bounding box and the object annotated with 
    the [COLOR2] bounding box moving in a different direction during the video?",
    "In the video, does the object with the [COLOR1] bounding box move in a different 
    direction from the object with the [COLOR2] bounding box?",
    "Are the objects annotated with the [COLOR1] and [COLOR2] bounding boxes traveling in 
    different directions during the entire video?"
]
\end{lstlisting}
\end{figure*}

\begin{figure*}[t]
\begin{lstlisting}[basicstyle=\ttfamily\small, backgroundcolor = \color{lightgray}, keywordstyle = {\textbf}, caption={\textbf{Answer templates for Movement Direction Comparison.}}, label={list:mdc_a}, breaklines=true]
movement_direction_comparison_true_positive_answers = [
    "Yes, the object annotated with the [COLOR1] bounding box is moving in the same 
    direction as the object annotated with the [COLOR2] bounding box throughout the video.",
    "Indeed, the object annotated with the [COLOR1] bounding box is heading in the same 
    direction as the object annotated with the [COLOR2] bounding box during the entire 
    video.",
    "Correct, the object annotated with the [COLOR1] bounding box and the object annotated 
    with the [COLOR2] bounding box are moving in the same direction in the video."
]

movement_direction_comparison_true_negative_answers = [
    "No, the object annotated with the [COLOR1] bounding box is moving in the same 
    direction as the object annotated with the [COLOR2] bounding box throughout the video.",
    "Actually, the object annotated with the [COLOR1] bounding box is heading in the same 
    direction as the object annotated with the [COLOR2] bounding box during the entire 
    video.",
    "Incorrect, the object annotated with the [COLOR1] bounding box and the object 
    annotated with the [COLOR2] bounding box are moving in the same direction in the video."
]

movement_direction_comparison_false_positive_answers = [
    "No, the object annotated with the [COLOR1] bounding box is moving in a different 
    direction from the object annotated with the [COLOR2] bounding box throughout the 
    video.",
    "Actually, the object annotated with the [COLOR1] bounding box is heading in a 
    different direction from the object annotated with the [COLOR2] bounding box during 
    the entire video.",
    "Incorrect, the object annotated with the [COLOR1] bounding box and the object 
    annotated with the [COLOR2] bounding box are moving in a different direction in the 
    video."
]

movement_direction_comparison_false_negative_answers = [
    "Yes, the object annotated with the [COLOR1] bounding box is moving in a different 
    direction from the object annotated with the [COLOR2] bounding box throughout the 
    video.",
    "Indeed, the object annotated with the [COLOR1] bounding box is heading in a different 
    direction from the object annotated with the [COLOR2] bounding box during the entire 
    video.",
    "Correct, the object annotated with the [COLOR1] bounding box and the object annotated 
    with the [COLOR2] bounding box are moving in a different direction in the video."
]
\end{lstlisting}
\end{figure*}

==> Tables/templates/distance.tex <==
\begin{figure*}[t]
\begin{lstlisting}[basicstyle=\ttfamily\small, backgroundcolor = \color{lightgray}, caption={\textbf{QA templates for Traveled Distance.}}, keywordstyle = {\textbf}, label={list:td}, breaklines=true]
traveled_distance_common_prompt = f"""The video lasts for [SECONDS] seconds, and [FRAMES] 
frames are uniformly sampled from it. These frames are located at [SECOND1]s,[SECOND2]s,
[SECOND3]s, ... . Please answer the following questions related to this video.

There is an object annotated with a [COLOR] bounding box in the video.
"""

traveled_distance_questions = [
    "What is the total distance traveled by the given object in the video?",
    "Can you calculate the total distance covered by the object in the video?",
    "Tell me the overall distance the object has traveled in the video.",
    "Could you provide the total distance the object moved throughout the video?",
    "How much distance did the object travel during the entire video?",
    "Measure the distance the object traveled throughout the video.",
    "What is the total distance traveled by a given object from [START] seconds to [END] 
    seconds?",
    "Can you calculate the total distance the object traveled between [START] seconds and 
    [END] seconds?",
    "Tell me how far the object moved from [START] seconds to [END] seconds.",
    "Could you measure the total distance the object covered between [START] and [END] 
    seconds?",
    "How much distance did the object travel during the period from [START] to 
    [END] seconds?",
    "Provide the total distance traveled by the object between [START] and [END] seconds.",
]

traveled_distance_answers = [
    "The total distance traveled by the given object is [DISTANCE].",
    "The given object's traveled distance is [DISTANCE].",
    "The given object has traveled a total of [DISTANCE].",
    "The entire distance the given object traveled amounts to [DISTANCE].",
    "The given object moved a total distance of [DISTANCE].",
    "The distance traveled by the given object from [START] to [END] seconds is 
    [DISTANCE].",
    "The given object traveled [DISTANCE] between [START] and [END] seconds.",
    "From [START] to [END] seconds, the given object moved a distance of [DISTANCE].",
    "The distance the given object moved from [START] to [END] seconds is [DISTANCE].",
    "Between [START] and [END] seconds, the given object traveled a total of [DISTANCE]."
]
\end{lstlisting}
\end{figure*}




==> Tables/templates/distance_comparison.tex <==
\begin{figure*}[t]
\begin{lstlisting}[basicstyle=\ttfamily\small, backgroundcolor = \color{lightgray}, keywordstyle = {\textbf}, caption={\textbf{Question templates for Traveled Distance Comparison.}}, label={list:tdc_q}, breaklines=true]
traveled_distance_comparison_common_prompt = f"""The video lasts for [SECONDS] seconds, 
and [FRAMES] frames are uniformly sampled from it. These frames are located at [SECOND1]s,
[SECOND2]s,[SECOND3]s, ... . Please answer the following questions related to this video.

There are two objects annotated with [COLOR1] and [COLOR2] bounding boxes in the video.
"""

traveled_distance_comparison_positive_questions = [
    "Which object travels a greater distance in the video: the one with the [COLOR1] 
    bounding box or the one with the [COLOR2] bounding box?",
    "Which object moves farther throughout the video, the object annotated with the [COLOR1] 
    bounding box or the [COLOR2] bounding box?",
    "Which object covers more distance in the video: the one annotated with the [COLOR1] 
    bounding box or the [COLOR2] bounding box?",
    "Between the objects annotated with the [COLOR1] and [COLOR2] bounding boxes, which one 
    moves a longer distance throughout the video?",
    "Between the two objects, one annotated with the [COLOR1] bounding box and the other 
    annotated with the [COLOR2] bounding box, which one moves farther during the entire 
    video?",
    "Which object, the one annotated with the [COLOR1] bounding box or the [COLOR2] 
    bounding box, has a greater travel distance in the video?"
]

traveled_distance_comparison_negative_questions = [
    "Which object travels a shorter distance in the video: the one with the [COLOR1] 
    bounding box or the one with the [COLOR2] bounding box?",
    "Which object moves a shorter distance throughout the video, the object annotated with 
    the [COLOR1] bounding box or the [COLOR2] bounding box?",
    "Which object covers less distance in the video: the one annotated with the [COLOR1]
    bounding box or the [COLOR2] bounding box?",
    "Between the objects annotated with the [COLOR1] and [COLOR2] bounding boxes, which one 
    moves a shorter distance throughout the video?",
    "Between the two objects, one annotated with the [COLOR1] bounding box and the other 
    annotated with the [COLOR2] bounding box, which one moves less during the entire 
    video?",
    "Which object, the one annotated with the [COLOR1] bounding box or the [COLOR2] 
    bounding box, has a shorter travel distance in the video?"
]
\end{lstlisting}
\end{figure*}


\begin{figure*}[t]
\begin{lstlisting}[basicstyle=\ttfamily\small, backgroundcolor = \color{lightgray}, keywordstyle = {\textbf}, caption={\textbf{Answer templates for Traveled Distance Comparison.}}, label={list:tdc_a}, breaklines=true]
traveled_distance_comparison_positive_answers = [
    "The object annotated with the [COLOR1] bounding box has traveled a greater distance 
    than the object annotated with the [COLOR2] bounding box throughout the video.",
    "In the video, the object annotated with the [COLOR1] bounding box has moved a greater 
    distance than the one annotated with the [COLOR2] bounding box.",
    "The object annotated with the [COLOR1] bounding box covers more distance throughout 
    the video compared to the object annotated with the [COLOR2] bounding box.",
    "During the entire video, the distance traveled by the object annotated with the 
    [COLOR1] bounding box is greater than that of the object annotated with the
    [COLOR2] bounding box.",
    "In the video, the object annotated with the [COLOR1] bounding box has traveled farther 
    than the object annotated with the [COLOR2] bounding box."
]

traveled_distance_comparison_negative_answers = [
    "The object annotated with the [COLOR1] bounding box has traveled a shorter distance 
    than the object annotated with the [COLOR2] bounding box throughout the video.",
    "In the video, the object annotated with the [COLOR1] bounding box has moved a shorter 
    distance than the one annotated with the [COLOR2] bounding box.",
    "The object annotated with the [COLOR1] bounding box covers less distance throughout the 
    video compared to the object annotated with the [COLOR2] bounding box.",
    "During the entire video, the distance traveled by the object annotated with the 
    [COLOR1] bounding box is less than that of the object annotated with the [COLOR2] 
    bounding box.",
    "In the video, the object annotated with the [COLOR1] bounding box has traveled a 
    shorter distance than the object annotated with the [COLOR2] bounding box."
]
\end{lstlisting}
\end{figure*}

==> Tables/templates/speed.tex <==
\begin{figure*}[t]
\begin{lstlisting}[basicstyle=\ttfamily\small, backgroundcolor = \color{lightgray}, keywordstyle = {\textbf}, caption={\textbf{QA templates for Traveling Speed.}}, label={list:ts}, breaklines=true]
traveling_speed_common_prompt = f"""The video lasts for [SECONDS] seconds, and [FRAMES] 
frames are uniformly sampled from it. These frames are located at [SECOND1]s,[SECOND2]s,
[SECOND3]s, ... . Please answer the following questions related to this video.

There is an object annotated with a [COLOR] bounding box in the video.
"""

traveling_speed_questions = [
    "What is the average speed of the given object in the video?",
    "Calculate the average speed of the object in the video.",
    "Tell me the object's average speed throughout the video.",
    "Could you provide the average velocity of the object throughout the video?",
    "What is the object's average speed during the video?",
    "Can you measure the average speed for the object in the entire video?",
    "What is the average speed of the given object from [START] seconds to [END] seconds?",
    "Can you calculate the average speed of the object between [START] and [END] seconds?",
    "Tell me the object's average speed from [START] to [END] seconds.",
    "Could you provide the average velocity of the object during the time period from 
    [START] to [END] seconds?",
    "What is the average speed of the object between [START] and [END] seconds?",
    "Measure the object's average velocity during the interval from [START] to [END] 
    seconds?"
]

traveling_speed_answers = [
    "The average speed of the given object is [SPEED] throughout the video.",
    "The object's average speed across the entire video is [SPEED].",
    "Throughout the video, the object moves at an average speed of [SPEED].",
    "The given object maintains an average speed of [SPEED] during the entire video.",
    "The average velocity of the given object throughout the video is [SPEED].",
    "The average speed of the given object from [START] to [END] seconds is [SPEED].",
    "The object's average speed between [START] and [END] seconds is [SPEED].",
    "From [START] to [END] seconds, the object moves at an average speed of [SPEED].",
    "The given object has an average velocity of [SPEED] during the time period from 
    [START] to [END] seconds.",
    "The object's average speed from [START] to [END] seconds is [SPEED]."
]
\end{lstlisting}
\end{figure*}

==> Tables/templates/speed_comparison.tex <==
\begin{figure*}[t]
\begin{lstlisting}[basicstyle=\ttfamily\small, backgroundcolor = \color{lightgray}, keywordstyle = {\textbf}, caption={\textbf{Question templates for Traveling Speed Comparison.}}, label={list:tsc_q}, breaklines=true]
traveling_speed_comparison_common_prompt = f"""The video lasts for [SECONDS] seconds, 
and [FRAMES] frames are uniformly sampled from it. These frames are located at [SECOND1]s,
[SECOND2]s,[SECOND3]s, ... . Please answer the following questions related to this video.

There are two objects annotated with [COLOR1] and [COLOR2] bounding boxes in the video.
"""

traveling_speed_comparison_positive_questions = [
    "Which object moves at a higher speed in the video: the one with the [COLOR1] bounding 
    box or the one with the [COLOR2] bounding box?",
    "Which object moves faster throughout the video, the object annotated with the [COLOR1] 
    bounding box or the [COLOR2] bounding box?",
    "Which object maintains a greater speed in the video: the one annotated with the 
    [COLOR1] bounding box or the [COLOR2] bounding box?",
    "Between the objects annotated with the [COLOR1] and [COLOR2] bounding boxes, which one 
    moves at a higher speed throughout the video?",
    "Between the two objects, one annotated with the [COLOR1] bounding box and the other 
    with the [COLOR2] bounding box, which one has a higher speed during the entire video?",
    "Which object, the one annotated with the [COLOR1] bounding box or the [COLOR2] 
    bounding box, has a greater average speed in the video?",
]

traveling_speed_comparison_negative_questions = [
    "Which object moves at a lower speed in the video: the one with the [COLOR1] bounding 
    box or the one with the [COLOR2] bounding box?",
    "Which object moves more slowly throughout the video, the object annotated with the 
    [COLOR1] bounding box or the [COLOR2] bounding box?",
    "Which object maintains a slower speed in the video: the one annotated with the [COLOR1] 
    bounding box or the [COLOR2] bounding box?",
    "Between the objects annotated with the [COLOR1] and [COLOR2] bounding boxes, which one 
    moves at a slower speed throughout the video?",
    "Between the two objects, one annotated with the [COLOR1] bounding box and the other 
    with the [COLOR2] bounding box, which one has a slower speed during the entire video?",
    "Which object, the one annotated with the [COLOR1] bounding box or the [COLOR2] 
    bounding box, has a lower average speed in the video?"
]
\end{lstlisting}
\end{figure*}


\begin{figure*}[t]
\begin{lstlisting}[basicstyle=\ttfamily\small, backgroundcolor = \color{lightgray}, keywordstyle = {\textbf}, caption={\textbf{Answer templates for Traveling Speed Comparison.}}, label={list:tsc_a}, breaklines=true]
traveling_speed_comparison_postivie_answers = [
    "The object annotated with the [COLOR1] bounding box has moved at a faster speed than 
    the object annotated with the [COLOR2] bounding box throughout the video.",
    "In the video, the object annotated with the [COLOR1] bounding box moves faster than 
    the one annotated with the [COLOR2] bounding box.",
    "The object annotated with the [COLOR1] bounding box maintains a higher speed 
    throughout the video compared to the object annotated with the [COLOR2] bounding box.",
    "During the entire video, the speed of the object annotated with the [COLOR1] bounding 
    box is greater than that of the object annotated with the [COLOR2] bounding box.",
    "In the video, the object annotated with the [COLOR1] bounding box has moved faster 
    than the object annotated with the [COLOR2] bounding box.",
]

traveling_speed_comparison_negative_answers = [ 
    "The object annotated with the [COLOR1] bounding box has moved at a slower speed than 
    the object annotated with the [COLOR2] bounding box throughout the video.",
    "In the video, the object annotated with the [COLOR1] bounding box moves more slowly 
    than the one annotated with the [COLOR2] bounding box.",
    "The object annotated with the [COLOR1] bounding box maintains a lower speed throughout 
    the video compared to the object annotated with the [COLOR2] bounding box.",
    "During the entire video, the speed of the object annotated with the [COLOR1] bounding 
    box is less than that of the object annotated with the [COLOR2] bounding box.",
    "In the video, the object annotated with the [COLOR1] bounding box has moved more 
    slowly than the object annotated with the [COLOR2] bounding box."
]
\end{lstlisting}
\end{figure*}

==> Tables/templates/timestamp.tex <==
\begin{figure*}[t]
\begin{lstlisting}[basicstyle=\ttfamily\small, backgroundcolor = \color{lightgray}, keywordstyle = {\textbf}, caption={\textbf{QA templates for Direction Timestamp.}}, label={list:dt}, breaklines=true]
direction_timestamp_common_prompt = f"""The video lasts for [SECONDS] seconds, and [FRAMES] 
frames are uniformly sampled from it. These frames are located at [SECOND1]s,[SECOND2]s,
[SECOND3]s, ... . Please answer the following questions related to this video.

There is an object annotated with a [COLOR] bounding box in the video.
"""

direction_timestamp_questions = [
    "Describe the timestamp when the object moves in the [CLOCK] o'clock direction.",
    "Can you provide the moment when the object moves in the [CLOCK] o'clock direction?",
    "Explain the time at which the object heads toward the [CLOCK] o'clock direction.",
    "At what timestamp does the object start moving in the [CLOCK] o'clock direction?",
    "When does the object begin traveling in the [CLOCK] o'clock direction?"
]

direction_timestamp_answers = [
    "The given object is heading toward the [CLOCK] o'clock direction from [START] to [END] 
    seconds.",
    "The object moves in the direction of [CLOCK] o'clock between [START] and [END] 
    seconds.",
    "From [START] to [END] seconds, the object is heading toward the [CLOCK] o'clock 
    direction.",
    "The object is traveling toward the [CLOCK] o'clock direction during the time period 
    from [START] to [END] seconds.",
    "Between [START] and [END] seconds, the object moves toward the [CLOCK] o'clock 
    direction."
]
\end{lstlisting}
\end{figure*}

==> sec/0_abstract.tex <==
\begin{abstract}
The ABSTRACT is to be in fully justified italicized text, at the top of the left-hand column, below the author and affiliation information.
Use the word ``Abstract'' as the title, in 12-point Times, boldface type, centered relative to the column, initially capitalized.
The abstract is to be in 10-point, single-spaced type.
Leave two blank lines after the Abstract, then begin the main text.
Look at previous \confName abstracts to get a feel for style and length.
\end{abstract}

==> sec/1_intro.tex <==
\section{Introduction}
\label{sec:intro}

Please follow the steps outlined below when submitting your manuscript to the IEEE Computer Society Press.
This style guide now has several important modifications (for example, you are no longer warned against the use of sticky tape to attach your artwork to the paper), so all authors should read this new version.

%-------------------------------------------------------------------------
\subsection{Language}

All manuscripts must be in English.

\subsection{Dual submission}

Please refer to the author guidelines on the \confName\ \confYear\ web page for a
discussion of the policy on dual submissions.

\subsection{Paper length}
Papers, excluding the references section, must be no longer than eight pages in length.
The references section will not be included in the page count, and there is no limit on the length of the references section.
For example, a paper of eight pages with two pages of references would have a total length of 10 pages.
{\bf There will be no extra page charges for \confName\ \confYear.}

Overlength papers will simply not be reviewed.
This includes papers where the margins and formatting are deemed to have been significantly altered from those laid down by this style guide.
Note that this \LaTeX\ guide already sets figure captions and references in a smaller font.
The reason such papers will not be reviewed is that there is no provision for supervised revisions of manuscripts.
The reviewing process cannot determine the suitability of the paper for presentation in eight pages if it is reviewed in eleven.

%-------------------------------------------------------------------------
\subsection{The ruler}
The \LaTeX\ style defines a printed ruler which should be present in the version submitted for review.
The ruler is provided in order that reviewers may comment on particular lines in the paper without circumlocution.
If you are preparing a document using a non-\LaTeX\ document preparation system, please arrange for an equivalent ruler to appear on the final output pages.
The presence or absence of the ruler should not change the appearance of any other content on the page.
The camera-ready copy should not contain a ruler.
(\LaTeX\ users may use options of \texttt{iccv.sty} to switch between different versions.)

Reviewers:
note that the ruler measurements do not align well with lines in the paper --- this turns out to be very difficult to do well when the paper contains many figures and equations, and, when done, looks ugly.
Just use fractional references (\eg, this line is $087.5$), although in most cases one would expect that the approximate location will be adequate.


\subsection{Paper ID}
Make sure that the Paper ID from the submission system is visible in the version submitted for review (replacing the ``*****'' you see in this document).
If you are using the \LaTeX\ template, \textbf{make sure to update paper ID in the appropriate place in the tex file}.


\subsection{Mathematics}

Please number all of your sections and displayed equations as in these examples:
\begin{equation}
  E = m\cdot c^2
  \label{eq:important}
\end{equation}
and
\begin{equation}
  v = a\cdot t.
  \label{eq:also-important}
\end{equation}
It is important for readers to be able to refer to any particular equation.
Just because you did not refer to it in the text does not mean some future reader might not need to refer to it.
It is cumbersome to have to use circumlocutions like ``the equation second from the top of page 3 column 1''.
(Note that the ruler will not be present in the final copy, so is not an alternative to equation numbers).
All authors will benefit from reading Mermin's description of how to write mathematics:
\url{http://www.pamitc.org/documents/mermin.pdf}.

\subsection{Blind review}

Many authors misunderstand the concept of anonymizing for blind review.
Blind review does not mean that one must remove citations to one's own work---in fact it is often impossible to review a paper unless the previous citations are known and available.

Blind review means that you do not use the words ``my'' or ``our'' when citing previous work.
That is all.
(But see below for tech reports.)

Saying ``this builds on the work of Lucy Smith [1]'' does not say that you are Lucy Smith;
it says that you are building on her work.
If you are Smith and Jones, do not say ``as we show in [7]'', say ``as Smith and Jones show in [7]'' and at the end of the paper, include reference 7 as you would any other cited work.

An example of a bad paper just asking to be rejected:
\begin{quote}
\begin{center}
    An analysis of the frobnicatable foo filter.
\end{center}

   In this paper we present a performance analysis of our previous paper [1], and show it to be inferior to all previously known methods.
   Why the previous paper was accepted without this analysis is beyond me.

   [1] Removed for blind review
\end{quote}


An example of an acceptable paper:
\begin{quote}
\begin{center}
     An analysis of the frobnicatable foo filter.
\end{center}

   In this paper we present a performance analysis of the  paper of Smith \etal [1], and show it to be inferior to all previously known methods.
   Why the previous paper was accepted without this analysis is beyond me.

   [1] Smith, L and Jones, C. ``The frobnicatable foo filter, a fundamental contribution to human knowledge''. Nature 381(12), 1-213.
\end{quote}

If you are making a submission to another conference at the same time, which covers similar or overlapping material, you may need to refer to that submission in order to explain the differences, just as you would if you had previously published related work.
In such cases, include the anonymized parallel submission~\cite{Authors14} as supplemental material and cite it as
\begin{quote}
[1] Authors. ``The frobnicatable foo filter'', F\&G 2014 Submission ID 324, Supplied as supplemental material {\tt fg324.pdf}.
\end{quote}

Finally, you may feel you need to tell the reader that more details can be found elsewhere, and refer them to a technical report.
For conference submissions, the paper must stand on its own, and not {\em require} the reviewer to go to a tech report for further details.
Thus, you may say in the body of the paper ``further details may be found in~\cite{Authors14b}''.
Then submit the tech report as supplemental material.
Again, you may not assume the reviewers will read this material.

Sometimes your paper is about a problem which you tested using a tool that is widely known to be restricted to a single institution.
For example, let's say it's 1969, you have solved a key problem on the Apollo lander, and you believe that the 1970 audience would like to hear about your
solution.
The work is a development of your celebrated 1968 paper entitled ``Zero-g frobnication: How being the only people in the world with access to the Apollo lander source code makes us a wow at parties'', by Zeus \etal.

You can handle this paper like any other.
Do not write ``We show how to improve our previous work [Anonymous, 1968].
This time we tested the algorithm on a lunar lander [name of lander removed for blind review]''.
That would be silly, and would immediately identify the authors.
Instead write the following:
\begin{quotation}
\noindent
   We describe a system for zero-g frobnication.
   This system is new because it handles the following cases:
   A, B.  Previous systems [Zeus et al. 1968] did not  handle case B properly.
   Ours handles it by including a foo term in the bar integral.

   ...

   The proposed system was integrated with the Apollo lunar lander, and went all the way to the moon, don't you know.
   It displayed the following behaviours, which show how well we solved cases A and B: ...
\end{quotation}
As you can see, the above text follows standard scientific convention, reads better than the first version, and does not explicitly name you as the authors.
A reviewer might think it likely that the new paper was written by Zeus \etal, but cannot make any decision based on that guess.
He or she would have to be sure that no other authors could have been contracted to solve problem B.
\medskip

\noindent
FAQ\medskip\\
{\bf Q:} Are acknowledgements OK?\\
{\bf A:} No.  Leave them for the final copy.\medskip\\
{\bf Q:} How do I cite my results reported in open challenges?
{\bf A:} To conform with the double-blind review policy, you can report results of other challenge participants together with your results in your paper.
For your results, however, you should not identify yourself and should not mention your participation in the challenge.
Instead present your results referring to the method proposed in your paper and draw conclusions based on the experimental comparison to other results.\medskip\\

\begin{figure}[t]
  \centering
  \fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
   %\includegraphics[width=0.8\linewidth]{egfigure.eps}

   \caption{Example of caption.
   It is set in Roman so that mathematics (always set in Roman: $B \sin A = A \sin B$) may be included without an ugly clash.}
   \label{fig:onecol}
\end{figure}

\subsection{Miscellaneous}

\noindent
Compare the following:\\
\begin{tabular}{ll}
 \verb'$conf_a$' &  $conf_a$ \\
 \verb'$\mathit{conf}_a$' & $\mathit{conf}_a$
\end{tabular}\\
See The \TeX book, p165.

The space after \eg, meaning ``for example'', should not be a sentence-ending space.
So \eg is correct, {\em e.g.} is not.
The provided \verb'\eg' macro takes care of this.

When citing a multi-author paper, you may save space by using ``et alia'', shortened to ``\etal'' (not ``{\em et.\ al.}'' as ``{\em et}'' is a complete word).
If you use the \verb'\etal' macro provided, then you need not worry about double periods when used at the end of a sentence as in Alpher \etal.
However, use it only when there are three or more authors.
Thus, the following is correct:
   ``Frobnication has been trendy lately.
   It was introduced by Alpher~\cite{Alpher02}, and subsequently developed by
   Alpher and Fotheringham-Smythe~\cite{Alpher03}, and Alpher \etal~\cite{Alpher04}.''

This is incorrect: ``... subsequently developed by Alpher \etal~\cite{Alpher03} ...'' because reference~\cite{Alpher03} has just two authors.

\begin{figure*}
  \centering
  \begin{subfigure}{0.68\linewidth}
    \fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
    \caption{An example of a subfigure.}
    \label{fig:short-a}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.28\linewidth}
    \fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
    \caption{Another example of a subfigure.}
    \label{fig:short-b}
  \end{subfigure}
  \caption{Example of a short caption, which should be centered.}
  \label{fig:short}
\end{figure*}


==> sec/2_formatting.tex <==
\section{Formatting your paper}
\label{sec:formatting}

All text must be in a two-column format.
The total allowable size of the text area is $6\frac78$ inches (17.46 cm) wide by $8\frac78$ inches (22.54 cm) high.
Columns are to be $3\frac14$ inches (8.25 cm) wide, with a $\frac{5}{16}$ inch (0.8 cm) space between them.
The main title (on the first page) should begin 1 inch (2.54 cm) from the top edge of the page.
The second and following pages should begin 1 inch (2.54 cm) from the top edge.
On all pages, the bottom margin should be $1\frac{1}{8}$ inches (2.86 cm) from the bottom edge of the page for $8.5 \times 11$-inch paper;
for A4 paper, approximately $1\frac{5}{8}$ inches (4.13 cm) from the bottom edge of the
page.

%-------------------------------------------------------------------------
\subsection{Margins and page numbering}

All printed material, including text, illustrations, and charts, must be kept
within a print area $6\frac{7}{8}$ inches (17.46 cm) wide by $8\frac{7}{8}$ inches (22.54 cm)
high.
%
Page numbers should be in the footer, centered and $\frac{3}{4}$ inches from the bottom of the page.
The review version should have page numbers, yet the final version submitted as camera ready should not show any page numbers.
The \LaTeX\ template takes care of this when used properly.



%-------------------------------------------------------------------------
\subsection{Type style and fonts}

Wherever Times is specified, Times Roman may also be used.
If neither is available on your word processor, please use the font closest in
appearance to Times to which you have access.

MAIN TITLE.
Center the title $1\frac{3}{8}$ inches (3.49 cm) from the top edge of the first page.
The title should be in Times 14-point, boldface type.
Capitalize the first letter of nouns, pronouns, verbs, adjectives, and adverbs;
do not capitalize articles, coordinate conjunctions, or prepositions (unless the title begins with such a word).
Leave two blank lines after the title.

AUTHOR NAME(s) and AFFILIATION(s) are to be centered beneath the title
and printed in Times 12-point, non-boldface type.
This information is to be followed by two blank lines.

The ABSTRACT and MAIN TEXT are to be in a two-column format.

MAIN TEXT.
Type main text in 10-point Times, single-spaced.
Do NOT use double-spacing.
All paragraphs should be indented 1 pica (approx.~$\frac{1}{6}$ inch or 0.422 cm).
Make sure your text is fully justified---that is, flush left and flush right.
Please do not place any additional blank lines between paragraphs.

Figure and table captions should be 9-point Roman type as in \cref{fig:onecol,fig:short}.
Short captions should be centred.

\noindent Callouts should be 9-point Helvetica, non-boldface type.
Initially capitalize only the first word of section titles and first-, second-, and third-order headings.

FIRST-ORDER HEADINGS.
(For example, {\large \bf 1. Introduction}) should be Times 12-point boldface, initially capitalized, flush left, with one blank line before, and one blank line after.

SECOND-ORDER HEADINGS.
(For example, { \bf 1.1. Database elements}) should be Times 11-point boldface, initially capitalized, flush left, with one blank line before, and one after.
If you require a third-order heading (we discourage it), use 10-point Times, boldface, initially capitalized, flush left, preceded by one blank line, followed by a period and your text on the same line.

%-------------------------------------------------------------------------
\subsection{Footnotes}

Please use footnotes\footnote{This is what a footnote looks like.
It often distracts the reader from the main flow of the argument.} sparingly.
Indeed, try to avoid footnotes altogether and include necessary peripheral observations in the text (within parentheses, if you prefer, as in this sentence).
If you wish to use a footnote, place it at the bottom of the column on the page on which it is referenced.
Use Times 8-point type, single-spaced.


%-------------------------------------------------------------------------
\subsection{Cross-references}

For the benefit of author(s) and readers, please use the
{\small\begin{verbatim}
  \cref{...}
\end{verbatim}}  command for cross-referencing to figures, tables, equations, or sections.
This will automatically insert the appropriate label alongside the cross-reference as in this example:
\begin{quotation}
  To see how our method outperforms previous work, please see \cref{fig:onecol} and \cref{tab:example}.
  It is also possible to refer to multiple targets as once, \eg~to \cref{fig:onecol,fig:short-a}.
  You may also return to \cref{sec:formatting} or look at \cref{eq:also-important}.
\end{quotation}
If you do not wish to abbreviate the label, for example at the beginning of the sentence, you can use the
{\small\begin{verbatim}
  \Cref{...}
\end{verbatim}}
command. Here is an example:
\begin{quotation}
  \Cref{fig:onecol} is also quite important.
\end{quotation}

%-------------------------------------------------------------------------
\subsection{References}

List and number all bibliographical references in 9-point Times, single-spaced, at the end of your paper.
When referenced in the text, enclose the citation number in square brackets, for
example~\cite{Authors14}.
Where appropriate, include page numbers and the name(s) of editors of referenced books.
When you cite multiple papers at once, please make sure that you cite them in numerical order like this \cite{Alpher02,Alpher03,Alpher05,Authors14b,Authors14}.
If you use the template as advised, this will be taken care of automatically.

\begin{table}
  \centering
  \begin{tabular}{@{}lc@{}}
    \toprule
    Method & Frobnability \\
    \midrule
    Theirs & Frumpy \\
    Yours & Frobbly \\
    Ours & Makes one's heart Frob\\
    \bottomrule
  \end{tabular}
  \caption{Results.   Ours is better.}
  \label{tab:example}
\end{table}

%-------------------------------------------------------------------------
\subsection{Illustrations, graphs, and photographs}

All graphics should be centered.
In \LaTeX, avoid using the \texttt{center} environment for this purpose, as this adds potentially unwanted whitespace.
Instead use
{\small\begin{verbatim}
  \centering
\end{verbatim}}
at the beginning of your figure.
Please ensure that any point you wish to make is resolvable in a printed copy of the paper.
Resize fonts in figures to match the font in the body text, and choose line widths that render effectively in print.
Readers (and reviewers), even of an electronic copy, may choose to print your paper in order to read it.
You cannot insist that they do otherwise, and therefore must not assume that they can zoom in to see tiny details on a graphic.

When placing figures in \LaTeX, it's almost always best to use \verb+\includegraphics+, and to specify the figure width as a multiple of the line width as in the example below
{\small\begin{verbatim}
   \usepackage{graphicx} ...
   \includegraphics[width=0.8\linewidth]
                   {myfile.pdf}
\end{verbatim}
}


%-------------------------------------------------------------------------
\subsection{Color}

Please refer to the author guidelines on the \confName\ \confYear\ web page for a discussion of the use of color in your document.

If you use color in your plots, please keep in mind that a significant subset of reviewers and readers may have a color vision deficiency; red-green blindness is the most frequent kind.
Hence avoid relying only on color as the discriminative feature in plots (such as red \vs green lines), but add a second discriminative feature to ease disambiguation.

==> sec/3_finalcopy.tex <==
\section{Final copy}

You must include your signed IEEE copyright release form when you submit your finished paper.
We MUST have this form before your paper can be published in the proceedings.

Please direct any questions to the production editor in charge of these proceedings at the IEEE Computer Society Press:
\url{https://www.computer.org/about/contact}.
